RaFe: Ranking Feedback Improves Query Rewriting for RAG

As Large Language Models (LLMs) and Retrieval Augmentation Generation (RAG) techniques have evolved, query rewriting has been widely incorporated into the RAG system for downstream tasks like open-domain QA. Many works have attempted to utilize small models with reinforcement learning rather than costly LLMs to improve query rewriting. However, current methods require annotations (e.g., labeled relevant documents or downstream answers) or predesigned rewards for feedback, which lack generalization, and fail to utilize signals tailored for query rewriting. In this paper, we propose ours, a framework for training query rewriting models free of annotations. By leveraging a publicly available reranker, ours~provides feedback aligned well with the rewriting objectives. Experimental results demonstrate that ours~can obtain better performance than baselines.

==> tab/LLM_rewrite_prompt.tex <==
\begin{table}[ht]
\centering
\resizebox{1.0 \columnwidth}{!}{
\begin{tabular}{p{1.3\linewidth}}
\toprule
\textbf{Prompt}  \\
\midrule
Please provide a rewrite to express the same query based on the given query. Here are some example\\
\\
Query: what state is this zip code 85282?\\
Output: Which state corresponds to the zip code 85282?\\
\\
Query: why is gibbs model of reflection good\\
Output: What makes the Gibbs reflective cycle a beneficial model?\\
\\
Query: what does a thousand pardons means\\
Output: How is the phrase "a thousand pardons" interpreted?\\
\\
Query: what is a macro warning\\
Output: What does the term "macro warning" refer to?\\
\\
Query: \{\}\\
Output:\\
\bottomrule
\end{tabular}
}
\caption{The few-shot prompt for LLM-Rewrite when generating pseudo documents from LLMs.}
\label{tab:llm_rewrite_prompt}
\end{table}

==> tab/Query2doc_rewrite_prompt.tex <==
\begin{table}[ht]
\centering
\resizebox{1.0 \columnwidth}{!}{
\begin{tabular}{p{1.3\linewidth}}
\toprule
\textbf{Prompt}  \\
\midrule
Please provide a rewrite to express the same query based on the given query. Here are some example\\
\\
Query: what state is this zip code 85282?\\
Output: Welcome to TEMPE, AZ 85282. 85282 is a rural zip code in Tempe, Arizona. The population is primarily white, and mostly single. At \$200,200 the average home value here is a bit higher than average for the Phoenix-Mesa-Scottsdale metro area, so this probably isn’t the place to look for housing bargains.5282 Zip code is located in the Mountain time zone at 33 degrees latitude (Fun Fact: this is the same latitude as Damascus, Syria!) and -112 degrees longitude.\\
\\
Query: why is gibbs model of reflection good\\
Output: In this reflection, I am going to use Gibbs (1988) Reflective Cycle. This model is a recognised framework for my reflection. Gibbs (1988) consists of six stages to complete one cycle which is able to improve my nursing practice continuously and learning from the experience for better practice in the future.n conclusion of my reflective assignment, I mention the model that I chose, Gibbs (1988) Reflective Cycle as my framework of my reflective. I state the reasons why I am choosing the model as well as some discussion on the important of doing reflection in nursing practice.\\
\\
Query: what does a thousand pardons means\\
Output: Oh, that’s all right, that’s all right, give us a rest; never mind about the direction, hang the direction - I beg pardon, I beg a thousand pardons, I am not well to-day; pay no attention when I soliloquize, it is an old habit, an old, bad habit, and hard to get rid of when one’s digestion is all disordered with eating food that was raised forever and ever before he was born; good land! a man can’t keep his functions regular on spring chickens thirteen hundred years old.\\
\\
Query: what is a macro warning\\
Output: Macro virus warning appears when no macros exist in the file in Word. When you open a Microsoft Word 2002 document or template, you may receive the following macro virus warning, even though the document or template does not contain macros: C:\textbackslash<path>\textbackslash<file name>contains macros. Macros may contain viruses.\\
\\
Query: \{\}\\
Output:\\
\bottomrule
\end{tabular}
}
\caption{The few-shot prompt for Query2Doc when generating pseudo documents from LLMs adopted from \cite{query2doc}.}
\label{tab:query2doc_rewrite_prompt}
\end{table}

==> tab/freshqa_tab.tex <==

\begin{table}[ht]
\centering
\resizebox{1 \columnwidth}{!}{
\begin{tabular}{c|ccccc}
\toprule
\textbf{Methods} & \textbf{Fast} & \textbf{Slow} & \textbf{Never} & \textbf{False} & \textbf{Ave} \\
\midrule
QR                       & \textbf{40.15}           & 66.13             & 82.26             & 58.93             & 61.87             \\
LLM-Rewrite              & 21.26                    & 54.84             & 80.64             & 51.37             & 52.03             \\
Query2Doc                & 31.50                    & 58.87             & 79.84             & 52.43             & 55.66             \\
SFT$_{(T_{\text{sft}})}$ & 37.01                    & 69.36             & 82.26             & 60.63             & 60.63             \\
SFT$_{(T_{\text{all}})}$ & 40.16                    & 66.94             & 80.80             & 52.51             & 60.47             \\
ReFe$_{(KTO)}$           & 39.37                    & \textbf{70.16}    & \textbf{84.68}    & \textbf{54.09}    & \textbf{62.07}    \\
\bottomrule
\end{tabular}
}
\caption{The results of knowledge-changing questions. We list the result of English Freshqa. \textbf{Fast, Slow, Never} mean changing fast, slowly, and never changing. \textbf{False} indicates False-Premise, which means the wrong premise questions. }
% \vspace{-6mm}
\label{tab:freshqa}
\end{table}


==> tab/old/case_tab_1.tex <==
\begin{table}[ht]
\centering
\resizebox{1.0 \columnwidth}{!}{
\begin{tabular}{p{1.0\linewidth}}
\toprule
\textbf{Example 1}  \\
\midrule
Query: What is the birds name from Lion King. \\
\\
Rewrite Good: \\Identify the \textbf{bird character} from Lion King. \\\\
Rewrite Bad: \\What is the \underline{feathered friend} in the Lion King? \\
\midrule
\textbf{Example 2}  \\
\midrule
Query: An `Oryx' is what kind of animal? \\
\\
Rewrite Good: \\What \textbf{category of} animal does Oryx belong to?  \\\\
Rewrite Bad: \\Identify the \underline{animal kingdom} of an Oryx. \\
\bottomrule
\end{tabular}
}
\caption{Two examples of good-bad rewrite pairs, each contains an original query (Query) and two rewrites (Rewrite Good and Rewrite Bad).}
\label{tab:case_1}
\end{table}

==> tab/old/llm_feedback.tex <==
\begin{table}[ht]
\centering
\resizebox{1 \columnwidth}{!}{
\begin{tabular}{l|cc|cc}
\toprule
\textbf{Methods} & \textbf{Feedback} & \textbf{Annotation} & \textbf{FreshQa} & \textbf{Webqa}  \\
\midrule
OQR                       
&   -      &  -
&48.45     &  92.03 \\

SFT$_{(T_{\text{all}})}$  
&   -      &  -
&46.65     &  91.86  \\
LLM$_{(DPO)}$             
&   LLM    & yes 
&  49.61   &  92.10  \\
LLM$_{(KTO)}$    
&   LLM    & yes 
&  49.93   &  \textbf{92.75} \\
RaFe$_{(DPO)}$   
& Reranker & no 
& \textbf{50.89} &  \underline{92.69}  \\
RaFe$_{(KTO)}$   
& Reranker & no
& \underline{50.61} &  92.46           \\
\bottomrule
\end{tabular}
}
\caption{Results compared with LLMs feedback under \textsc{Expand} setting, SFT$_{DPO}$ indicates that first training with SFT on $T_{\text{sft}}$ and then training on $T_{\text{f}}$ with DPO.}
% \vspace{-6mm}
\label{tab:llm_feedback}
\end{table}

==> tab/old/main_tabel.tex <==

% \begin{table*}[ht]
% \centering
% % \LARGE
% \resizebox{2\columnwidth}{!}{
% \begin{tabular}{lc|cccc|cc}

% \toprule
% \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Base Model}} & \multicolumn{4}{c|}{\textbf{EN}} & \multicolumn{2}{c}{\textbf{ZH}} \\
% & & \textbf{FreshQA} & \textbf{NQ} & \textbf{TriviaQA} & \textbf{HotpotQA} & \textbf{FreshQA} & \textbf{WebQA} \\
% \midrule
% w/o retrieval            &   -                      & 43.03             & 49.86             & 62.85             & 39.32             & 38.51             & 85.95               \\
% OQR                      &   -                      & 61.01             & 55.51             & 66.31             & 47.40             & 48.45             & 92.03               \\
% \midrule
% \multicolumn{8}{c}{\textsc{Substitute}} \\
% \midrule
% LLM-Rewrite              & Qwen-max                 & 52.03             & 51.11             & 65.32             & 46.28             & \underline{49.82} & 91.63               \\
% Query2Doc                & Qwen-max                 & 55.56             & 51.41             & 63.98             & 46.17             & 49.41             & \textbf{92.49}      \\
% SFT$_{(T_{\text{sft}})}$ & Qwen-7b                  & 60.62             & 54.65             & 65.82             & 45.94             & 46.77             & 90.67               \\
% SFT$_{(T_{\text{all}})}$ & Qwen-7b                  & 60.46             & 54.24             & 65.87             & 46.02             & 44.44             & 90.27               \\
% RaFe$_{(PPO)}$           & SFT$_{(T_{\text{sft}})}$ & \underline{61.25} & 54.23             & 65.62             & 47.23             & 48.07             & \underline{91.75}   \\
% RaFe$_{(DPO)}$           & SFT$_{(T_{\text{sft}})}$ & 61.08             & 54.71             & \textbf{66.62}    & \textbf{47.75}    & 47.95             & 91.67               \\
% RaFe$_{(KTO)}$           & SFT$_{(T_{\text{sft}})}$ & \textbf{62.07}    & 55.01             & 66.03             & \underline{47.55} & \textbf{50.95}    & 91.57               \\
% \midrule
% \multicolumn{8}{c}{\textsc{Expand}} \\
% \midrule
% LLM-Rewrite              & Qwen-max                 & 61.10             & 54.85             & 66.63             & 48.33             & 49.40             & 92.23               \\
% Query2Doc                & Qwen-max                 & 61.18             & 53.71             & 66.30             & 48.12             & 48.30             & 92.29               \\
% SFT$_{(T_{\text{sft}})}$ & Qwen-7b                  & 59.83             & 55.32             & 66.63             & 49.11             & 48.05             & 91.25               \\
% SFT$_{(T_{\text{all}})}$ & Qwen-7b                  & 61.64             & 55.07             & 66.59             & 49.18             & 48.69             & 91.86               \\
% RaFe$_{(PPO)}$           & SFT$_{(T_{\text{sft}})}$ & \textbf{62.88}    & 55.40             & 66.64             & \underline{49.24} & 49.41             & 92.66               \\
% RaFe$_{(DPO)}$           & SFT$_{(T_{\text{sft}})}$ & 62.12             & \underline{55.60} & \underline{66.85} & 48.75             & \textbf{50.89}    & \textbf{92.69}      \\
% RaFe$_{(KTO)}$           & SFT$_{(T_{\text{sft}})}$ & \underline{62.41} & \textbf{55.65}    & \textbf{67.16}    & \textbf{49.33}    & \underline{50.61} & \underline{92.46}   \\
% \bottomrule
% \end{tabular}
% }
% \caption{The results on English and Chinese QA datasets with Top-5 documents.}
% % \vspace{-6mm}
% \label{tab:maintable}
% \end{table*}


==> tab/old/main_table_en.tex <==

\begin{table*}[ht]
\centering
% \LARGE
\resizebox{2.05\columnwidth}{!}{
\begin{tabular}{l|cccc|cccc|cccc|cccc}

\toprule
\multirow{3}{*}[-0.5em]{\textbf{Method}} & \multicolumn{4}{c|}{\textbf{FreshQA}} & \multicolumn{4}{c|}{\textbf{NQ}} & \multicolumn{4}{c|}{\textbf{TriviaQA}} & \multicolumn{4}{c}{\textbf{HotpotQA}} \\
\cmidrule{2-17}
& \multicolumn{2}{c}{raw} & \multicolumn{2}{c|}{ranked} & \multicolumn{2}{c}{raw} & \multicolumn{2}{c|}{ranked} & \multicolumn{2}{c}{raw} & \multicolumn{2}{c|}{ranked} & \multicolumn{2}{c}{raw} & \multicolumn{2}{c}{ranked} \\
\cmidrule{2-17} 
& EM & Prec@5 & EM & Prec@5 & EM & Prec@5 & EM & Prec@5 & EM & Prec@5 & EM & Prec@5 & EM & Prec@5 & EM & Prec@5 \\

\midrule
w/o retrieval                 
& 41.70 & - & - & -     
& 43.74 & - & - & -     
& 62.85  & - & - & - 
& 47.40 & - & - & -   
\\

OQR                 
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & -     
& 62.85  & - & - & - 
& 47.40 & - & - & -   
\\
\midrule
\multicolumn{17}{c}{\textsc{Substitute}} \\
\midrule

LLM-Rewrite                  
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & -     
& 62.85  & - & - & - 
& 47.40 & - & - & -   
\\

Query2Doc                  
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & -     
& 62.85  & - & - & - 
& 47.40 & - & - & -   
\\

SFT$_{(T_{\text{sft}})}$                   
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & -     
& 62.85  & - & - & - 
& 47.40 & - & - & -   
\\

SFT$_{(T_{\text{all}})}$                
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & -     
& 62.85  & - & - & - 
& 47.40 & - & - & -   
\\

RaFe$_{(PPO)}$                 
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & -     
& 62.85  & - & - & - 
& 47.40 & - & - & -   
\\

RaFe$_{(DPO)}$                  
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & -     
& 62.85  & - & - & - 
& 47.40 & - & - & -   
\\

RaFe$_{(KTO)}$                   
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & -     
& 62.85  & - & - & - 
& 47.40 & - & - & -   
\\

\midrule
\multicolumn{17}{c}{\textsc{Expand}} \\
\midrule

LLM-Rewrite                  
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & -     
& 62.85  & - & - & - 
& 47.40 & - & - & -   
\\

Query2Doc                  
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & -     
& 62.85  & - & - & - 
& 47.40 & - & - & -   
\\

SFT$_{(T_{\text{sft}})}$                   
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & -     
& 62.85  & - & - & - 
& 47.40 & - & - & -   
\\

SFT$_{(T_{\text{all}})}$                
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & -     
& 62.85  & - & - & - 
& 47.40 & - & - & -   
\\

RaFe$_{(PPO)}$                 
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & -     
& 62.85  & - & - & - 
& 47.40 & - & - & -   
\\

RaFe$_{(DPO)}$                  
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & -     
& 62.85  & - & - & - 
& 47.40 & - & - & -   
\\

RaFe$_{(KTO)}$                   
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & -     
& 62.85  & - & - & - 
& 47.40 & - & - & -   
\\

\bottomrule
\end{tabular}
}
\caption{The results on English and Chinese QA datasets with Top-5 documents.}
% \vspace{-6mm}
\label{tab:maintable}
\end{table*}

% online offline标注





% \begin{table*}[ht]
% \centering
% % \LARGE
% \resizebox{2\columnwidth}{!}{
% \begin{tabular}{lc|cccc|cc}

% \toprule
% \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Base Model}} & \multicolumn{4}{c|}{\textbf{EN}} & \multicolumn{2}{c}{\textbf{ZH}} \\
% & & \textbf{FreshQA} & \textbf{NQ} & \textbf{TriviaQA} & \textbf{HotpotQA} & \textbf{FreshQA} & \textbf{WebQA} \\
% \midrule
% w/o retrieval            &   -                      & 43.03             & 49.86             & 62.85             & 39.32             & 38.51             & 85.95               \\
% OQR                      &   -                      & 61.01             & 55.51             & 66.31             & 47.40             & 48.45             & 92.03               \\
% \midrule
% \multicolumn{8}{c}{\textsc{Substitute}} \\
% \midrule
% LLM-Rewrite              & Qwen-max                 & 52.03             & 51.11             & 65.32             & 46.28             & \underline{49.82} & 91.63               \\
% Query2Doc                & Qwen-max                 & 55.56             & 51.41             & 63.98             & 46.17             & 49.41             & \textbf{92.49}      \\
% SFT$_{(T_{\text{sft}})}$ & Qwen-7b                  & 60.62             & 54.65             & 65.82             & 45.94             & 46.77             & 90.67               \\
% SFT$_{(T_{\text{all}})}$ & Qwen-7b                  & 60.46             & 54.24             & 65.87             & 46.02             & 44.44             & 90.27               \\
% RaFe$_{(PPO)}$           & SFT$_{(T_{\text{sft}})}$ & \underline{61.25} & 54.23             & 65.62             & 47.23             & 48.07             & \underline{91.75}   \\
% RaFe$_{(DPO)}$           & SFT$_{(T_{\text{sft}})}$ & 61.08             & 54.71             & \textbf{66.62}    & \textbf{47.75}    & 47.95             & 91.67               \\
% RaFe$_{(KTO)}$           & SFT$_{(T_{\text{sft}})}$ & \textbf{62.07}    & 55.01             & 66.03             & \underline{47.55} & \textbf{50.95}    & 91.57               \\
% \midrule
% \multicolumn{8}{c}{\textsc{Expand}} \\
% \midrule
% LLM-Rewrite              & Qwen-max                 & 61.10             & 54.85             & 66.63             & 48.33             & 49.40             & 92.23               \\
% Query2Doc                & Qwen-max                 & 61.18             & 53.71             & 66.30             & 48.12             & 48.30             & 92.29               \\
% SFT$_{(T_{\text{sft}})}$ & Qwen-7b                  & 59.83             & 55.32             & 66.63             & 49.11             & 48.05             & 91.25               \\
% SFT$_{(T_{\text{all}})}$ & Qwen-7b                  & 61.64             & 55.07             & 66.59             & 49.18             & 48.69             & 91.86               \\
% RaFe$_{(PPO)}$           & SFT$_{(T_{\text{sft}})}$ & \textbf{62.88}    & 55.40             & 66.64             & \underline{49.24} & 49.41             & 92.66               \\
% RaFe$_{(DPO)}$           & SFT$_{(T_{\text{sft}})}$ & 62.12             & \underline{55.60} & \underline{66.85} & 48.75             & \textbf{50.89}    & \textbf{92.69}      \\
% RaFe$_{(KTO)}$           & SFT$_{(T_{\text{sft}})}$ & \underline{62.41} & \textbf{55.65}    & \textbf{67.16}    & \textbf{49.33}    & \underline{50.61} & \underline{92.46}   \\
% \bottomrule
% \end{tabular}
% }
% \caption{The results on English and Chinese QA datasets with Top-5 documents.}
% % \vspace{-6mm}
% \label{tab:maintable}
% \end{table*}







==> tab/old/main_table_zh.tex <==
\begin{table}[ht]
\centering
% \LARGE
\resizebox{1\columnwidth}{!}{
\begin{tabular}{l|cccc|cccc}

\toprule
\multirow{3}{*}[-0.5em]{\textbf{Method}} & \multicolumn{4}{c|}{\textbf{FreshQA}} & \multicolumn{4}{c}{\textbf{WebQA}} \\
\cmidrule{2-9}
& \multicolumn{2}{c}{raw} & \multicolumn{2}{c|}{ranked} & \multicolumn{2}{c}{raw} & \multicolumn{2}{c}{ranked} \\
\cmidrule{2-9} 
& EM & Prec@5 & EM & Prec@5 & EM & Prec@5 & EM & Prec@5  \\

\midrule
w/o retrieval                 
& 41.70 & - & - & -     
& 43.74 & - & - & -   
\\

OQR                 
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & -  
\\
\midrule
\multicolumn{9}{c}{\textsc{Substitute}} \\
\midrule

LLM-Rewrite                  
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & -    
\\

Query2Doc                  
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & -   
\\

SFT$_{(T_{\text{sft}})}$                   
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & -  
\\

SFT$_{(T_{\text{all}})}$                
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & - 
\\

RaFe$_{(PPO)}$                 
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & -   
\\

RaFe$_{(DPO)}$                  
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & -   
\\

RaFe$_{(KTO)}$                   
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & -   
\\

\midrule
\multicolumn{9}{c}{\textsc{Expand}} \\
\midrule

LLM-Rewrite                  
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & -    
\\

Query2Doc                  
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & -   
\\

SFT$_{(T_{\text{sft}})}$                   
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & -  
\\

SFT$_{(T_{\text{all}})}$                
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & - 
\\

RaFe$_{(PPO)}$                 
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & -   
\\

RaFe$_{(DPO)}$                  
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & -   
\\

RaFe$_{(KTO)}$                   
& 62.27 & 27.48 & 62.56 & 30.88     
& 43.74 & - & - & -   
\\

\bottomrule
\end{tabular}
}
\caption{The results on Chinese QA datasets with Top-5 documents.}
% \vspace{-6mm}
\label{tab:maintable_zh}
\end{table}


==> tab/old/rewrite_num.tex <==

\begin{table}[ht]
\centering
\resizebox{0.85 \columnwidth}{!}{
\begin{tabular}{c|cccc}
\toprule
\multirow{2}{*}{\textbf{Nums}} & \multicolumn{2}{c}{\textbf{Raw}}    & \multicolumn{2}{c}{\textbf{Ranked}} \\ 
& EM & Prec@5 & EM & Prec@5 \\
\midrule
0 
& 61.87        & 27.48   
& 62.56        & 30.88    \\
1      
& 61.89        & 28.00   
& 63.06        & 33.32    \\
2      
& 62.65        & \underline{28.50}   
& \textbf{64.85} & \underline{34.72}    \\
3      
& 62.07        & \textbf{28.70}   
& 63.78        & 34.56    \\
4      
& \textbf{63.61}        & 28.26   
& 64.20        & \textbf{35.00}    \\
5      
& \underline{63.38}        & 28.46   
& \underline{64.32}        & 34.68    \\
\bottomrule
\end{tabular}
}
\caption{The results of different rewrite nums in \textsc{Expand} setting. We list the result from 0 to 5 rewrites. The rewrites are generate by RaFe$_{(\text{KTO})}$.}
% \vspace{-6mm}
\label{tab:rewrite_num}
\end{table}

==> tab/old/topk_table.tex <==

\begin{table}[ht]
\centering
\resizebox{1 \columnwidth}{!}{
\begin{tabular}{c|ccccc}
\toprule
\textbf{Methods} & \textbf{Top-1} & \textbf{Top-3} & \textbf{Top-5} & \textbf{Top-10}  \\
\midrule
OQR                      & \textbf{53.86}     & 59.06             & 61.01             & 64.16               \\
% LLM-Rewrite              & 61.10             & 54.85             & --.--             & --.--               \\
% Query2Doc                & 61.18             & 53.71             & --.--             & --.--               \\
% SFT$_{(T_{\text{sft}})}$ & 59.83             & 55.32             & 66.63             & 49.11               \\
SFT$_{(T_{\theta})}$     & 53.58             & 58.64              & 60.64             & 64.03               \\
ReFe$_{(PPO)}$           & \underline{53.63} & \underline{59.28}  & \underline{61.25} & \textbf{65.43}      \\
ReFe$_{(DPO)}$           & 52.95             & 58.27              & 61.08             & 63.30               \\
ReFe$_{(KTO)}$           & 53.04             & \textbf{60.41}     & \textbf{62.07}    & \underline{65.15}   \\
\bottomrule
\end{tabular}
}
\caption{The results under \textsc{Substitute} setting on Freshqa with different number of documents.}
% \vspace{-6mm}
\label{tab:topk}
\end{table}
